An Analytic Approach to BCFT$_d$

We develop an analytic approach to Boundary Conformal Field Theory (BCFT), focussing on the two-point function of a general pair of scalar primary operators. The resulting crossing equation can be thought of as a vector equation in an infinite-dimensional space ${\cal V}$ of analytic functions of a single complex variable. We argue that in a unitary theory, functions in ${\cal V}$ satisfy a boundedness condition in the Regge limit. We identify a useful basis for ${\cal V}$, consisting of bulk and boundary conformal blocks with scaling dimensions which appear in OPEs of the mean field theory correlator. Our main achievement is an explicit expression for the action of the dual basis (the basis of liner functionals on ${\cal V}$) on an arbitrary conformal block. The practical merit of our basis is that it trivializes the study of perturbations around mean field theory. Our results are equivalent to a BCFT version of the Polyakov bootstrap. Our derivation of the expressions for the functionals relies on the identification of the Polyakov blocks with (suitably improved) boundary and bulk Witten exchange diagrams in $AdS_{d+1}$. We also provide another conceptual perspective on the Polyakov block expansion and the associated functionals, by deriving a new Lorentzian OPE inversion formula for BCFT.

==> sections/Checks.tex <==
%!TEX root = ../bcft_polyakov_draft.tex



\section{Some Checks of the Analytic Functionals}

==> sections/Discussion.tex <==
%!TEX root = ../bcft_polyakov_draft.tex


\section{Discussion and Outlook}




==> sections/Functionals_Polyakov.tex <==
%!TEX root = ../bcft_polyakov_draft.tex


\section{From Functionals to Polyakov Blocks, and Back}

Logic of the section:

1) Restrict to ``physical'' space of functions ${\cal V}$, which comes equipped with a notion of topology (convergence). Such functions should be complex analytic in the appropriate domain, with singularities
of physical 2pt functions, and suitable boundedness at infinity.
Below we will propose a precise mathematical characterization of this space, but our results will not depend crucially on that mathematical formulation. 

2) Bulk and Neumann boundary double-trace blocks are a basis of this space, up to a single linear relation that arises from the existence of the basic contact Witten diagram (which belongs to ${\cal V}$). Alternatively,
bulk and Dirichlet boundary double-trace blocks, with no relation. In this work, we will focus on the former choice.

3) Define a basis of ${\cal V}^*$ as the functionals  dual to this primal basis.  (By definition, one can commute the action of these functionals with infinite sums that converge in ${\cal V}$).

4) Define the bulk and boundary Polyakov blocks in terms of their direct channel expansion, and prove their crossed channel expansion. By construction, one can rewrite the OPE decomposition in terms of a sum over over bulk + boundary Polyakov blocks.

5) Polyakov blocks can be characterized abstractly as {\it the} functions in ${\cal V}$ with this type of block decomposition in both channels. Easy to show that they are unique.

6) God (=Witten) handed us functions with precisely these properties: Witten exchanges  = Polyakov blocks. We can then read off the action of the functionals on conformal blocks from the coefficients in front of the double-traces in the conformal block expansion of the Witten exchanges. This is a well-defined technical problem that we will solve in the next section.

7) The mathematically precise formulation of ${\cal V}$ that we conjecturally put forward is that ${\cal V}$ is   the $\ell^1$ Banach space of the $w$-plane expansion (after removing the bulk and boundary identity singularities). Comment here on the $z \to \infty$ condition (or perhaps discuss it at the beginning of the section).  One can check that all blocks are in $\ell^1$, all exhanges are in $\ell^1$, and the basic contact is in $\ell^1$.
By contrast, the ``Dirichlet'' contact with normal derivatives is {\it not} in $\ell^1$.

8) Perhaps comment at the end or before on space of BCFTs that interpolate between Neumann and Dirichlet, and how that fits conceptually in this framework.
